Instance Segmentation in 3D Scenes using Semantic Superpoint Tree Networks

Instance segmentation in 3D scenes is fundamental in many applications of scene understanding. It is yet challenging due to the compound factors of data irregularity and uncertainty in the numbers of instances. State-of-the-art methods largely rely on a general pipeline that first learns point-wise features discriminative at semantic and instance levels, followed by a separate step of point grouping for proposing object instances. While promising, they have the shortcomings that (1) the second step is not supervised by the main objective of instance segmentation, and (2) their point-wise feature learning and grouping are less effective to deal with data irregularities, possibly resulting in fragmented segmentations. To address these issues, we propose in this work an end-to-end solution of Semantic Superpoint Tree Network (SSTNet) for proposing object instances from scene points. Key in SSTNet is an intermediate, semantic superpoint tree (SST), which is constructed based on the learned semantic features of superpoints, and which will be traversed and split at intermediate tree nodes for proposals of object instances. We also design in SSTNet a refinement module, termed CliqueNet, to prune superpoints that may be wrongly grouped into instance proposals. Experiments on the benchmarks of ScanNet and S3DIS show the efficacy of our proposed method. At the time of submission, SSTNet ranks top on the ScanNet (V2) leaderboard, with 2% higher of mAP than the second best method. The source code in PyTorch is available at https://github.com/Gorilla-Lab-SCUT/SSTNet.

==> Schedule.tex <==
% \subsection{Problem}
% \label{Problem}
% \begin{itemize}
%     \item [1)]
%     The training process is also unstable. I've try to add batch norm or not.
%     \item [2)]
%     The current performance is still insufficient, the target \textbf{AP} is 50.
%     \item [3)]
%     When the classifier judges the node fusion, the depth of node maybe a important signal, in the next step, I should encode the depth signal to help model training.
%     \item [4)]
%     The final mask refinement will improve performance significantly, I try to concatenate the global feature after point-wise features for each proposal, then perform binary segmentation, but it doesn't work, maybe an MLP is poor.
%     \item [4)]
%     It's hard to end-to-end training as the current stage, it will cause out-of-memory and the time cost is high, now the backbone is frozen.
% \end{itemize}

\subsection{2021\_01\_04}
\label{DOING}
\begin{itemize}
    \item [1)] using the number of over-segmentation as a dimension of features, which caused no performance improvement, but stable.
    \item [2)] refinement(freeze the whole network and finetune the refinement network: mlp or gcn to realize binary segmentation):
        \begin{itemize}
            \item [a)] binary segment all points for each proposal(concat global features then mlp for each point). (fail, damage performance)
            \item [b)] binary segment all over-segmentation for each proposal(concat global features then mlp for each point). (No significant improvement, $AP48.1->AP48.2$)
            \item [c)] binary segment all over-segmentation for each proposal using graph convolutional network. (the same as $b)$)
        \end{itemize}
    \item [3)] Training end-to-end(split into 3 stages, need 1 week):
        \begin{itemize}
            \item [stage1)] training backbone to get semantic and offset(0-64)
            \item [stage2)] training merge\&split mlp together(64-128)
            \item [stage3)] training scorenet together(128-384)
        \end{itemize}
\end{itemize}



